The Highest Expected Reward Decoding for HMMs with Application to Recombination Detection

Hidden Markov models are traditionally decoded by the Viterbi algorithm which finds the highest probability state path in the model. In recent years, several limitations of the Viterbi decoding have been demonstrated, and new algorithms have been developed to address them \citep{Kall2005,Brejova2007,Gross2007,Brown2010}. In this paper, we propose a new efficient highest expected reward decoding algorithm (HERD) that allows for uncertainty in boundaries of individual sequence features. We demonstrate usefulness of our approach on jumping HMMs for recombination detection in viral genomes.

==> concl.tex <==
\section{Conclusion}

In this paper, we have introduced a novel decoding algorithm for
hidden Markov models seeking an annotation of the sequence
in which boundaries of individual sequence features are at least
approximately correct. This decoding is particularly appropriate in
situations where the exact boundaries are difficult to determine, and
perhaps their knowledge is not even necessary. 
%Our algorithm runs in
%time linear in the sequence length, although compared to the classical
%Viterbi and posterior decoding it will run a factor of $W$ slower for
%typical HMMs.

We apply our algorithm to the problem of recombination detection in
HIV genomes. Here, the Viterbi decoding considers for a
given annotation only a single alignment of the query to the profile HMMs
and only one placement of breakpoints. In contrast,
we marginalize the probabilities over all possible alignments and over nearby
placements of recombination boundaries. As a result, we are able to
predict individual recombinant regions with greater sensitivity and
specificity. 

Our experiments also suggest venues for future improvement. First of
all, the accuracy results vary with the choice of 
parameters $P_j$, $W$, and $\gamma$. 
It remains an open question how to choose these parameters
in a principled way. We have also observed that our algorithm does not
perform as well as the Viterbi algorithm in finding the exact
boundaries. Perhaps this could be solved by a gain function in which a
boundary with a more distant buddy gets a smaller score. Similarly,
our algorithm performs slightly worse in terms of base-level accuracy,
and this shortcoming perhaps could be addressed by adding a positive
score for every correctly colored nucleotide to the gain function.
In general, the framework of maximum expected gain decoding is very
promising, because it allows to tailor decoding algorithm for a specific 
application domain.

\paragraph{Acknowledgements.} We would like to thank Dan Brown
and Jakub Truszkowski for helpful discussion on related problems.
Research of TV and BB is funded
by European Community FP7 grants IRG-224885 and IRG-231025.


==> intro.tex <==
\section{Introduction}

Hidden Markov models (HMMs) are an important tool for modeling and
annotation of biological sequences and other data, such as
natural language texts. The goal of sequence annotation is to label
each symbol of the input sequence according to its meaning or
a function. For example, in gene finding, we seek to distinguish
regions of DNA that encode proteins from non-coding sequence.  An HMM
defines a probability distribution $\Pr(A|X)$ over all 
annotations $A$ of sequence $X$. Typically, one uses the
well-known Viterbi algorithm \citep{Forney1973} or its variants 
for more complex models \citep{Brejova2007} to find the annotation
with the highest overall probability $\arg\max_A Pr(A|X)$.  In this paper,
we design an efficient HMM decoding algorithm that finds the optimal 
annotation for a different optimization criterion that is
more appropriate in many applications. 

In recent years, several annotation strategies were shown to achieve
better performance than the Viterbi decoding in particular
applications \citep{Kall2005,Gross2007,Brown2010}. 
Generally, they can be expressed in the
terminology of \emph{gain functions} introduced in the context
of stochastic context-free grammars \citep{Hamada2009}. 
In particular, we choose a gain function
$G(A,A')$ which characterizes similarity between a proposed
annotation $A$ and the (unknown) correct annotation $A'$. The goal
is then to find the annotation $A$ with the highest expected value of
$G(A,A')$ over the distribution of $A'$ defined by the HMM
conditioning on sequence $X$. That is, we maximize
$E_{A'|X}[G(A,A')] = \sum_{A'} G(A,A')P(A'|X).$

In this framework, the Viterbi decoding optimizes the identity gain
function $G(A,A') = [A=A']$, that is the gain is 1 if we
predict the whole annotation exactly correctly and 0 otherwise. 
There may be many
high-probability annotations besides the optimal one, and they
are disregarded by this gain function, even though their consensus
may suggest a different answer that is perhaps
more accurate locally.
On the other hand, the posterior decoding \citep{Durbin1998}
predicts at each position a label that has the highest
posterior probability at that position, marginalizing over all annotations. 
Therefore it
optimizes the expected gain under the gain function that counts the
number of correctly predicted labels in $A$ with respect to $A'$.

These two gain functions are extremes: the Viterbi decoding
assigns a positive gain to the annotation only if it is completely
correct, while the posterior decoding gain function rewards every
correct label. It is often appropriate to consider gain
functions in between these two extremes. For example, in the
context of gene finding, \citet{Gross2007} use a gain function that
assigns a score +1 for each correctly predicted coding region boundary
and score $-\gamma$ for predicted boundary that is a false
positive. Indeed, one of the main objectives of gene finding is to
find exact positions of these boundaries, since even a small error
may change the predicted protein significantly.
Parameter $\gamma$ in the gain function controls the trade-off between
sensitivity and specificity.

While the coding region boundaries are well defined in gene
finding and it is desirable to locate them precisely, in other
applications, such as transmembrane protein topology prediction, we
only wish to infer the approximate locations of feature boundaries.
The main reason is that the underlying HMMs do not contain enough
information to locate the boundaries exactly, and there are typically many
annotations of similar probability with slightly different boundaries.
This issue was recently examined by \citet{Brown2010} in a Viterbi-like
setting, where we assign gain to an annotation, if all feature
boundaries in $A$ are within some distance $W$ from the corresponding
boundary in the correct annotation $A'$. Unfortunately, the problem
has to be addressed by heuristics, since it is 
NP-hard even for $W=0$.

In this paper, we propose a new gain function in which each feature
boundary in $A$ gets score +1 if it is within distance $W$ from the
corresponding boundary in $A'$, and score $-\gamma$ otherwise. Our
definition allows to consider nearby boundary positions as equivalent
as in \citet{Brown2010}, yet it avoids the requirement that the whole
annotation needs to be essentially correct to receive any gain at all.
Another benefit is that our gain function can be efficiently optimized
in time linear in the length of the input sequence.

We apply our algorithm to the problem of detecting recombination in
the genome of the human immunodeficiency virus (HIV) with 
jumping HMMs \citep{Schultz2006}. A jumping HMM
consists of a profile HMM \citep{Durbin1998} for each known subtype of
HIV. Recombination events are represented by a special jump
transitions between different profile HMMs. The goal is to
determine for a new HIV genome whether it comes from one of the
known subtypes or whether it is a recombination of several
subtypes. However, the exact position of a breakpoint can be
difficult to determine, particularly if the two recombining strains
were very similar near the recombination point. Our gain function
therefore corresponds very naturally to this problem. It scores
individual predicted recombination points but allows some tolerance in
their exact placement. 


